NNLO interpolation grids for jet production at the LHC

Fast interpolation-grid frameworks facilitate an efficient and flexible evaluation of higher-order predictions for any choice of parton distribution functions or value of the strong coupling $\alpha_s$. They constitute an essential tool for the extraction of parton distribution functions and Standard Model parameters, as well as studies of the dependence of cross sections on the renormalisation and factorisation scales. The APPLfast project provides a generic interface between the parton-level Monte Carlo generator NNLOJET and both the APPLgrid and the fastNLO libraries for the grid interpolation. The extension of the project to include hadron-hadron collider processes at next-to-next-to-leading order in perturbative QCD is presented, together with an application for jet production at the LHC.

==> applfast-preamble.tex <==
%!TEX root = applfast.tex

% Language and utf8 usage
\RequirePackage[british]{babel}%
\RequirePackage[utf8]{inputenc}

%% Additional latex packages
\RequirePackage{amsmath,amssymb,mathtools}
\RequirePackage{graphicx}%
\DeclareGraphicsExtensions{.pdf,.png,.jpg}%
\graphicspath{{./plots/}}%
\RequirePackage{multirow}%
\RequirePackage[usenames,x11names,svgnames,table]{xcolor}%
\RequirePackage{xspace}%
\RequirePackage{booktabs}%
\renewcommand{\arraystretch}{1.2} % make lines a bit larger for tables
\RequirePackage[citecolor=blue,linkcolor=blue,linktoc=page,urlcolor=blue,colorlinks=true]{hyperref}
\RequirePackage{cite}
\RequirePackage{arydshln}
\RequirePackage{siunitx}

% tikz
\RequirePackage{tikz}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{fit}
\usetikzlibrary{backgrounds}
\usetikzlibrary{calc}
% tikz defs
\newcommand{\colorrect}[1]{\tikz[baseline]{\path[fill=#1] (-0.1ex,-0.1ex) rectangle (1.5ex,1.5ex);}}
\newcommand{\nenode}[1]{(0.88,0.88) node[anchor=north east,shape=rectangle,fill=white, font=\scriptsize] {#1}}
\newcommand{\nenodee}[1]{(0.89,0.89) node[anchor=north east,shape=rectangle,fill=white, font=\scriptsize] {#1}}
\newcommand{\swnode}[1]{(0.14,0.16) node[anchor=south west,shape=rectangle,fill=white, font=\scriptsize] {#1}}
\newcommand{\swnodee}[1]{(0.16,0.16) node[anchor=south west,shape=rectangle,fill=white, font=\scriptsize] {#1}}
\newcommand{\nwnodee}[1]{(0.16,0.89) node[anchor=north west,shape=rectangle,fill=white, font=\scriptsize] {#1}}
\newcommand{\ttnode}[1]{(0.5,0.91) node[anchor=base, shape=rectangle, font=\large] {#1}}
% color defs for tikz usage
\definecolor{kgreen}{rgb}{0.0,0.6,0.5}
\definecolor{kblue}{rgb}{0.3,0.4,0.7}
\definecolor{kmgreen}{rgb}{0.5,0.7,0.2}
\definecolor{kyellow}{rgb}{1.0,0.9,0.0}
\definecolor{korange}{rgb}{0.9,0.6,0.1}
\definecolor{kbrown}{rgb}{0.7,0.5,0.2}
\definecolor{kred}{rgb}{0.6,0.1,0.1}
\definecolor{kpurple}{rgb}{0.6,0.1,0.5}
\definecolor{kcyan}{rgb}{0.1,0.7,0.9}
\definecolor{kblack}{rgb}{0.0,0.0,0.0}
\definecolor{xyellow}{rgb}{1.0,0.8,0}
\definecolor{xblue}{rgb}{0,0,0.6}
\definecolor{xgreen}{rgb}{0.2,0.8,0.2}
\definecolor{xred}{rgb}{0.6,0.0,0.0}
\definecolor{petrol}{rgb}{0.0,0.37,0.42}
% produce new external pdfs for the plots
%\usetikzlibrary{external}
%\tikzexternalize % activate!
% end of tikz

%\bibliographystyle{spphys}
\bibliographystyle{utphys}


\newcommand{\LO}{\text{LO}\xspace}
\newcommand{\NLO}{\text{NLO}\xspace}
\newcommand{\NNLO}{\text{NNLO}\xspace}
\newcommand{\NNLOJET}{\texorpdfstring{NNLO\protect\scalebox{0.8}{JET}}{NNLOJET}\xspace}

\newcommand{\rd}{\ensuremath{\mathrm{d}}}

\newcommand{\Pe}{{\ensuremath{\mathrm{e}}}\xspace}
\newcommand{\Pp}{{\ensuremath{\mathrm{p}}}\xspace}
\newcommand{\PZ}{{\ensuremath{\mathrm{Z}}}\xspace}
\newcommand{\PW}{{\ensuremath{\mathrm{W}}}\xspace}
\newcommand{\jet}{\text{jet}\xspace}

\newcommand{\murf}{\ensuremath{\mu_{\rm R/F}}\xspace}
\newcommand{\mur}{\ensuremath{\mu_{\rm R}}\xspace}
\newcommand{\muf}{\ensuremath{\mu_{\rm F}}\xspace}
\newcommand{\mufn}{\ensuremath{\mu_{{\rm F}_0}}\xspace}
\newcommand{\mup}{\ensuremath{\mu_{0}}\xspace}
\newcommand{\muref}{\ensuremath{\mu_\text{ref}}\xspace}

\newcommand{\xa}{\ensuremath{x_1}\xspace}
\newcommand{\xb}{\ensuremath{x_2}\xspace}
\newcommand{\sigab}{\ensuremath{\sigma_{ab}}\xspace}
\newcommand{\as}{\ensuremath{\alpha_{\mathrm{s}}}\xspace}
\newcommand{\asmz}{\ensuremath{\as(M_{\PZ})}\xspace}
\newcommand{\asmur}{\ensuremath{\as(\mur)}\xspace}
\newcommand{\tilmu}{\ensuremath{\tilde{\mu}}\xspace}
\newcommand{\kfactor}{\ensuremath{K}-factor\xspace}
\newcommand{\kfactors}{\ensuremath{K}-factors\xspace}

\newcommand{\chisq}{\ensuremath{\chi^{2}}\xspace}
\newcommand{\ndf}{\ensuremath{n_\mathrm{dof}}\xspace}
%\newcommand{\etajet}{\ensuremath{\eta_\mathrm{lab}^\mathrm{jet}}\xspace}
\newcommand{\ptjet}{\ensuremath{p^\mathrm{jet}_\mathrm{T}}\xspace}
\newcommand{\ptjetmin}{\ensuremath{p^\mathrm{jet}_\mathrm{T,min}}\xspace}
\newcommand{\htp}{\ensuremath{\hat{H}_\mathrm{T}}\xspace}
\newcommand{\etalab}{\ensuremath{\eta_\mathrm{lab}^\mathrm{jet}}\xspace}
\newcommand{\GeVsq}{\ensuremath{\mathrm{GeV}^2}\xspace}
\newcommand{\GeV}{\ensuremath{\mathrm{GeV}}\xspace}
\newcommand{\TeV}{\ensuremath{\mathrm{TeV}}\xspace}
\newcommand{\pt}{\ensuremath{p_\mathrm{T}}\xspace}
\newcommand{\Qsq}{\ensuremath{Q^{2}}\xspace}

\providecommand{\ptavg}{\ensuremath{p_{\mathrm{T,avg}}}\xspace}
\providecommand{\ptoneb}{\ensuremath{p_{\mathrm{T},1}}\xspace}
\providecommand{\pttwob}{\ensuremath{p_{\mathrm{T},2}}\xspace}
\providecommand{\ystar}{\ensuremath{y^{*}}\xspace}
\providecommand{\yboost}{\ensuremath{y_{\mathrm{b}}}\xspace}

\providecommand{\yabs}{\ensuremath{\left|y\right|}\xspace}
\providecommand{\rbthm}{\rule[-2ex]{0ex}{5ex}}
\providecommand{\rbtrr}{\rule[-0.8ex]{0ex}{3.2ex}}

\providecommand{\XFITTER}{\textsc{xFitter}\xspace}
\providecommand{\HOPPET}{\textsc{Hoppet}\xspace}
\providecommand{\HERAFITTER}{\textsc{HERAFitter}\xspace}
\providecommand{\NLOJETPP}{\textsc{NLOJet++}\xspace}
\providecommand{\FASTNLO}{\textsc{fastNLO}\xspace}
\providecommand{\APPLGRID}{\textsc{APPLgrid}\xspace}
\providecommand{\APPLFAST}{\textsc{APPLfast}\xspace}
\providecommand{\PLOUGHSHARE}{\texttt{Ploughshare}\xspace}
\providecommand{\pp}{\ensuremath{\text{pp}}\xspace}
\providecommand{\kt}{\ensuremath{k_\text{T}}\xspace}
%\providecommand{\mjj}{\ensuremath{M_\text{jj}}\xspace}
\providecommand{\mjj}{\ensuremath{m_\text{12}}\xspace}
\providecommand{\ymax}{\ensuremath{y_{\text{max}}}\xspace}
\providecommand{\ptave}{\ensuremath{\langle p_\text{T1,2}\rangle}\xspace}
\providecommand{\chisqndof}{\ensuremath{\chi^2/n_\text{dof}}\xspace}
\providecommand{\ndof}{\ensuremath{n_\text{dof}}\xspace}
\providecommand{\ptmaxscl}{\ensuremath{\ptoneb\exp(0.3\,\ystar)}\xspace}


% %% DRAFT MODE
% \RequirePackage[mathlines]{lineno}%
% % \linenumbers
% \newcommand{\AHf}[1]{{\color{magenta}[#1]${}_\text{AH}$}\xspace}
% \newcommand{\DBf}[1]{{\color{blue}[#1]${}_\text{DB}$}\xspace}
% \newcommand{\DS}[1]{{\color{petrol}[#1]${}_\text{DS}$}\xspace}
% \newcommand{\MSf}[1]{{\color{purple}[#1]${}_\text{MS}$}\xspace}
% \newcommand{\KRf}[1]{{\color{violet}[#1]${}_\text{KR}$}\xspace}
% \newcommand{\CGf}[1]{{\color{orange}[#1]${}_\text{CG}$}\xspace}
% \newcommand{\KR}[1]{\footnote{{\color{violet}KR: #1}}}
% \newcommand{\MS}[1]{\footnote{{\color{purple}MS: #1}}}
% \newcommand{\DB}[1]{\footnote{{\color{blue}DB: #1}}}
% \newcommand{\AH}[1]{\footnote{{\color{magenta}AH: #1}}}
% \newcommand{\CG}[1]{\footnote{{\color{orange}CG: #1}}}
% % \newcommand{\KR}[1]{\footnote{\color{violet}[KR: #1]}}
% \providecommand{\TODO}[1]{{\noindent\textcolor{red}{\sffamily{\bfseries{}TODO:} #1}}}


